Canonical connections on sub-Riemannian manifolds with constant symbol

As a tool to address the equivalence problem in sub-Riemannian geometry, we introduce a canonical choice of grading and compatible affine connection, available on any sub-Riemannian manifold with constant symbol. We completely compute these structures for contact manifolds of constant symbol, including the cases where the connections of Tanaka-Webster-Tanno are not defined. We also give an original intrinsic grading on sub-Riemannian (2,3,5)-manifolds, and use this to present the first flatness theorem in this setting.

==> Engel234.tex <==
\section{The structure of $(2,3,4)$ manifolds}
Let $(M,E,g)$ be sub-Riemannian manifold with growth vector $\mathfrak{G} = (2,3,4)$. Then this submanifold will have a constant symbol, as there is only one choice of Cartan algebra called the Engel algebra. The algebra is given as
$$\mathfrak{g}_- = \mathfrak{g}_{-3} \oplus \mathfrak{g}_{-2} \oplus \mathfrak{g}_{-1}= \spn\{C\} \oplus \spn \{ B\} \oplus \spn \{ A_1, A_2 \},$$
where $A_1, A_2$ is an orthonormal basis, and where the only non-zero brackets are
$$[A_1, A_2] = B, \qquad [A_1, B] = C.$$
For this structure, we verify that $\mathfrak{g}_0 = 0$.

Let us introduce a grading on $(M,E,g)$ defined as follows. Working locally, we may assume that $E$ is trivial and oriented. Define $J: E \to E$ such that $u, Ju$ is positively oriented orthonormal basis for any for any unit vector $u$. Introduce a decomposition $E= E(0) \oplus E(1)$ such that $E(0)$ is defined as the kernel of the map $E\to TM/E^{-2}$, $X \mapsto [X,[X,JX]]$, and $E(1)$ is its orthogonal complement. If $X_0$ and $X_1$ are unit vector field spanning respectively $E(0)$ and $E(1)$, we define and $E$-grading $I$ by
$$(TM)_{-2} = \spn \{ [X_0, X_1]\}, \qquad (TM)_{-3} = ([X_1,[X_0, X_1]]).$$
We then observe that the decomposition $TM = E(0) \oplus E(1) \oplus (TM)_{-2} \oplus (TM)_{-3}$ does not depend on any of our local choices and hence makes sense globally. Furthermore, the taming metric $g_I$ of $E$ makes the previous decomposition orthonormal.

\begin{proposition}
For any $(2,3,4)$-sub-Riemannian metric, we have that the Morimoto grading $I$ given as above and the Morimoto connection $\nabla$ is the unique connection compatible with $g_I$ and such that the decomposition $TM = E(0) \oplus E(1) \oplus (TM)_{-2} \oplus (TM)_{-3}$ is parallel.
\end{proposition}

\begin{proof}
Since $\mathfrak{g}_0 =0$, the condition \eqref{Rcond} is void. As for condition \eqref{Tcond}, working locally, we write
$$E(0) \oplus E(1) \oplus (TM)_{-2} \oplus (TM)_{-3} = \spn \{X_0\} \oplus \spn\{ X_1\} \oplus \spn\{ Z_{-2}\}\oplus \spn\{Z_{-3}\},$$
with all vectors being unit vector fields and with $[X_0, X_1] = Z_{-2} \mod E$ and $[X_1, [X_0, X_1]] = Z_{-3} \mod E^{-2}$. We then see that
\begin{align*}
\langle T(\chi_I(Z_{-2})), X_0 \rangle & = \langle T(X_0, X_1), X_0 \rangle =  - \tr_{TM} \langle T_\times Z_{-2} , \mathbb{T}_\times X_0 \rangle
\end{align*}
\end{proof}


==> Free36.tex <==
\section{Example: Free Group and manifolds of maximal growth vector}
\subsection{Three dimensional case}
Consider the special case of sub-Riemannian manifolds with growth vector $(3,6)$. Such sub-Riemannian manifolds always have constant symbol. Let $X_1, X_2, X_3$ be an arbitrary local orthonormal basis and define $Z_{ij} = [X_i, X_j]$. Define a cross product on $E$, by
$$X_1 \times X_2 = X_3, \qquad X_2 \times X_3 = X_1, \qquad X_3 \times X_1 = X_2.$$
The unique selector of $E$ is then given by $\chi(Z_{ij}) = X_i \wedge X_j$. Write $\hat Z_{ij} = Z_{ij} - \pr_E Z_{ij}$ and note that $\| Z_{ij} \|_{\bar{g}} = 1$.
For any $i,j$, define $D_{ij}$ as the unique section of $\mathfrak{s}_I$ satisfying $D_{jj} =0$ and for $i\neq j$, and for $k$ different from $i$ and $j$,
$$D_{ij}(X_i) = X_j, \qquad D_{ij}(X_j) = - X_i, \qquad D_{ij}(X_k) = 0.$$
This map then satisfies
$$D_{ij}(\hat Z_{ij}) =0, \qquad D_{ij}(\hat Z_{ik}) = \hat Z_{jk}, \qquad D_{ij}(\hat Z_{jk})= - \hat Z_{ik}.$$

We consider first the case of \eqref{Rrestriction}. We observe that
\begin{align*} 
0 & = \langle  T_{X_i} , D_{ij}  \rangle , \\
0 & = \langle  T_{X_k} , D_{ij}  \rangle , \\
\langle R(X_i, X_j) , D_{ij} \rangle & = \langle T_{\hat Z_{ij}} , D_{ij} \rangle , \\
\langle R(X_i, X_j) , D_{ik} \rangle & = \langle T_{\hat Z_{ij}} , D_{ik} \rangle , \\
\langle T(X_i, X_j), X_i \rangle & = - \tr_{TM}  \langle T(\times, \hat Z_{ij}) , \mathbb{T}(\times, X_i) \rangle \\
T(X_i, X_j) & =  - \hat Z_{ij} - \tr_{TM} \mathbb{T}_\times^* T_\times \hat Z_{ij} , 
\end{align*}



\begin{align*}
& 0 =  \langle R(\chi(X_i)), D_{ij} \rangle = \langle \mathbf{T}_{X_i}, D_{ij}\rangle \\
& = - \langle \mathbf{T}(X_i, X_j), X_i \rangle + \frac{1}{2} ( \langle \mathbf{T}(X_i, \hat Z_{ik}), \hat Z_{jk} \rangle-  \langle \mathbf{T}(X_i, \hat Z_{jk}), \hat Z_{ik} \rangle)
\end{align*}
and
\begin{align*}
& 0 =  \langle R(\chi(X_k)), D_{ij} \rangle = \langle \mathbf{T}_{X_k}, D_{ij}\rangle \\
& = \langle \mathbf{T}(X_k, X_i), X_j \rangle - \langle \mathbf{T}(X_k, X_j), X_i \rangle + \frac{1}{2} ( \langle \mathbf{T}(X_k, \hat Z_{ik}), \hat Z_{jk} \rangle-  \langle \mathbf{T}(X_k, \hat Z_{jk}), \hat Z_{ik} \rangle)
\end{align*}
We can then write these both as
\begin{align*}
& 0 = -\| v \times w\|^2 \langle \mathbf{T}(v, w), v \rangle + \frac{1}{2} ( \langle \mathbf{T}(v, \mathbb{T}(v, v\times w) ), \mathbb{T}(w, v\times w)  \rangle-  \langle \mathbf{T}(v, \mathbb{T}(w, v \times w)), \mathbb{T}(w, v \times w) \rangle)
\end{align*}
\begin{align*}
& 0 =\| w\|^2 ( \langle \mathbf{T}(w, u), v \rangle - \langle \mathbf{T}( w, v), u \rangle )+ \frac{1}{2} ( \langle \mathbf{T}(w , \mathbb{T}(u,w)), \mathbb{T}(v,w) \rangle-  \langle \mathbf{T}(w, \mathbb{T}(v,w) ), \mathbb{T}(u,w)  \rangle)
\end{align*}


==> Selectors.tex <==


\section{Selectors and partial connection} \label{sec:Selectors}
\subsection{Selectors and partial one-forms}
Let $\chi$ be the selector of an equiregular subbundle $E$ of step $s$. Then given information about a one-form along just the subbundle $E$ and knowing the value of the differential along the selector will give us a unique way of extending the partial data to a full one-form. The statement can be found below and can be deduced from \cite{CGJK19}.
\begin{lemma} \label{lemma:PartialForm}
Let $\beta$ be any one-form and let $\eta$ be any one-form vanishing on $E$. Then the unique solution $\alpha$ of the equations
\begin{equation} \label{AlphaSol} \alpha|_E = \beta|_E, \qquad \chi^* d\alpha = \eta,\end{equation}
is given by
\begin{align*}
\alpha & = (\id+ \chi^* d)^{s-1} \beta -  \sum_{j=0}^{s-2} \binom{s-1}{j+1} (\chi^* d)^j \eta  \\
& = \beta^\chi -  \frac{(\id -\chi^* d)^{s-1} - \id}{\chi^* d} \eta .
\end{align*}
\end{lemma}
We include a proof, since the formulation of the result is a bit different than in our reference.
\begin{proof}
{\it If $\eta =0$:} We note that $\chi^* d\beta$ is a one-form vanishing on $E$ so $(\id + \chi^*  d)^{s-1} \chi^* d\beta = 0$. Hence
$$\chi^* d (\id + \chi^* d)^{s-1} \beta  = (\id + \chi^* d)^{s-1} \chi^* d \beta =0,$$
and furthermore, we have $(\id + \chi^* d)^{s-1} \beta |E = \beta|E$.

{\it If $\beta =0$:} We note that then $\alpha$ vanishes on $E$, then $\alpha + \eta = (\id + \chi^* d) \alpha$ vanishes on $E^{-2}$. It follows that
\begin{align*}
0= & (\id +\chi^* d)^{s-2} (\alpha + \eta) = \sum_{j=0}^{s-2} \binom{s-2}{j} (\chi^* d)^j (\alpha + \eta)  \\
& = \alpha + \sum_{j=0}^{s-3} \binom{s-2}{j+1} (\chi^* d)^j \eta + \sum_{j=0}^{s-2} \binom{s-2}{j} (\chi^* d)^j \eta \\
& = \alpha + \sum_{j=0}^{s-2} \binom{s-1}{j+1} (\chi^* d)^j \eta 
\end{align*}

{\it The general case:} The general solution can be found by adding two previous equations.
\end{proof}

We also


\subsection{Selectors and partial connections}
In Lemma~\ref{lemma:PartialForm}, we can replace $d$ with any operator $L$ from one-forms to two-forms such that $(\id + \chi^* L)\alpha$ vanishes on $E^{-k-1}$ if $\alpha$ vanishes $E^{-k}$. This holds true also when the forms in question have values in a vector bundle. We will use this result for partial connections.

Let $\calA$ be any vector bundle and let $E$ be a subbundle of the tangent bundle. \emph{A partial connection} $\scrD$ on $\calA$ in the direction of $E$ is a map $\Gamma(E) \times \Gamma(\calA) \to \Gamma(\calA)$
$$(X, A) \mapsto \scrD_XA $$
which is tensorial in the first argument and satisfies $\scrD_X \phi A = (X\phi) A + \phi \scrD_X A$ for any $\phi \in C^\infty(M)$. We note the following result, which can also be deduced from \cite{CGJK19}.
\begin{lemma} \label{lemma:ChiUnique}
Let $\scrD$ be a partial connection be a connection on $\calA$ in the direction of~$E$.
\begin{enumerate}[\rm (a)]
\item Then there exists a unique affine connection~$\nabla = \scrD^\chi$ on~$\calA$, such that $\nabla_{|E} = \scrD$ and such that the curvature $R$ of $\nabla$ satisfies
$$R(\chi(\, \cdot \,)) = 0.$$
We also have $\Hol(\nabla) = \Hol(\scrD)$.
\item Let $\eta$ be a one-form vanishing on $E$ with values in $\End \calA$. Then there is a unique affine connection $\nabla$ such that $\nabla_{|E} = \scrD$ and such that its curvature $R$ satisfies
$$R(\chi(\, \cdot \,)) = \eta.$$
This connection is given by
$$\nabla_X Y = \scrD^\chi_X Y -  \sum_{j=0}^{s-2} \binom{s-1}{j+1} ((\chi^* d^{\scrD^\chi})^j \eta)(X)Y.$$
\end{enumerate}
\end{lemma}
\begin{proof}
Let $k$ be the rank of $\calA$. Consider the principal bundle
$$\GL(k) \to \GL(\calA) \stackrel{\pi}{\to} M.$$
Then a partial connection correspond to a partial form $\bomega: \pi_*^{-1} E \to \mathfrak{gl}(k)$ satisfying $\bomega(v \cdot a) = \Ad(a^{-1}) \bomega(v)$. Let $L: \Gamma(T^*\GL(\calA) \otimes \mathfrak{gl}(k)) \to \Gamma(\wedge^2 T^*\GL(\calA) \otimes \mathfrak{gl}(k))$ be the operator
$$L\alpha = d\alpha + \frac{1}{2} [\alpha, \alpha].$$
Let $\hat \omega : T\GL(\calA) \to \mathfrak{gl}(\calA)$ be any principal connection with $\hat \omega |_{\pi_*^{-1} E} = \bomega$. Write $\calH = \ker \omega$ and let $v \in T_{\pi(f)} M \mapsto h_f v \in \calH_{f}$ be the corresponding horizontal lift. Define a selector $\hat \chi$ of $\pi_*^{-1} E$ by
$$\hat \chi: h_f v \mapsto h_f \chi(v).$$
\begin{enumerate}[\rm (a)]
\item We define $\omega^\chi$ as the solution of
$$\omega^\chi = \bomega, \qquad \hat \chi^* L\omega^\chi = 0.$$
This has the the same holonomy by \cite{CGJK19}.
\item Introduce $\hat \eta \in \Gamma(T^*\GL(\calA) \otimes \mathfrak{gl}(k))$,
$$\hat \eta(w) = f^{-1} \eta(\pi_* w) f, \qquad w \in T_{f}P. $$
We define $\omega$,
$$\omega = \bomega, \qquad \hat \chi^* L \omega = \hat \eta.$$
The solution is
$$\omega = \omega^\chi -  \sum_{j=0}^{s-2} \binom{s-1}{j+1} (\hat \chi^* d)^j \hat \eta.$$
We finally observe that
$$\hat \chi^* d\hat \eta(w)= f^{-1} (\chi^* d^{\scrD^{\chi}} \eta)(\pi_* w) f.\qedhere$$ 

\end{enumerate}
\end{proof}


%\subsection{Partial connections on $E$ and complements}
%If we have a sub-Riemannian manifold $(M, E, g)$ with a chosen complement to $E$ or equivalently a chosen projection $\pr_E : TM \to E$, then it was observed in \cite[Lemma~2.9]{CGT19} that we have the following unique way of choosing a partial connection on $E$. For any partial connection $\mathscr{D}$, define its \emph{partial torsion} by
%$$\mathbf{t}(X,Y) = \mathscr{D}_X Y - \mathscr{D}_Y X - [X, Y], \qquad X, Y \in \Gamma(E),$$
%which takes values in $TM$.
%\begin{lemma} \label{lemma:PCUnique}
%Let $\pr_E: TM \to E$ be any projection. Then there is a unique partial connection $\scrD^0$ such that its partial torsion $\mathbf{t}^0$ satisfies $\pr_E\mathbf{t}^0(E,E) =0$. Furthermore, let $\scrD$ be any compatible partial connection on $E$ in the direction of $E$ with partial torsion $\mathbf{t}$. Define $\mathbf{t}_E$ by $\mathbf{t}_E(X,Y) = \pr_E \mathbf{t}(X,Y)$. Then for any $X,Y, Z \in \Gamma(E)$,
%\begin{align*}
%\langle (\scrD_X - \scrD_X^0) Y, Z \rangle & = \frac{1}{2} \langle \mathbf{t}_E(X, Y) ,Z \rangle_g - \frac{1}{2} \langle \mathbf{t}_E(Y,Z) , X \rangle_g - \frac{1}{2} \langle \mathbf{t}_E(X,Z), Y \rangle_g
%\end{align*}
%
%\end{lemma}
%Note that if we take any taming Riemannian metric $\tilde g$ of $g$ such that $\pr_E$ becomes the orthogonal projection, then we can write $\scrD^0$ as $\scrD_X Y = \pr_E \nabla_X^{\tilde g} Y$, $X, Y \in \Gamma(E)$ where $\nabla^{\tilde g}$ is the Levi-Civita connection of $\tilde g$. Using the Koszul formula for the Levi-Civita connection, we conclude that
%\begin{align*}
%\langle \scrD_X^0 Y, Z \rangle & = \frac{1}{2} \left( X\langle Y, Z \rangle_g + Y \langle X, Z \rangle_g - Z \langle X, Y \rangle_g  \right) \\
%& \qquad \frac{1}{2} \left( \langle \pr_E [X, Y], Z \rangle_g - \langle \pr_E [X, Z], Y \rangle_g - \langle \pr_E [Y,Z], X \rangle_g \right).
%\end{align*}



